A robust extension to the triple plane pressure mode matching method by filtering convective perturbations

Time-periodic CFD simulations are widely used to investigate turbomachinery components. The triple-plane pressure mode matching method (TPP) developed by Ovenden and Rienstra extracts the acoustic part in such simulations. Experience shows that this method is subject to significant errors when the amplitude of pseudo-sound is high compared to sound. Pseudo-sound are unsteady pressure fluctuations with a convective character. The presented extension to the TPP improves the splitting between acoustics and the rest of the unsteady flow field. The method is simple: i) the acoustic eigenmodes are analytically determined for a uniform mean flow as in the original TPP; ii) the suggested model for convective pressure perturbations uses the convective wavenumber as axial wavenumber and the same orthogonal radial shape functions as for the acoustic modes. The reliability is demonstrated on the simulation data of a low-pressure fan. As acoustic and convective perturbations are separated, the accuracy of the results increases close to sources, allowing a reduction of the computational costs by shortening the simulation domain. The extended method is as robust as the original one--giving the same results for the acoustic modes in absence of convective perturbations.

==> 7_figures.tex <==

%methods
\begin{figure}[hbt]
\begin{center}
%	\includegraphics[trim = 0mm 0mm 20mm 0mm, clip,
%	width=\columnwidth]{steadyFlowField_0.20.eps}
\caption{\label{steady_0.21}
Density and velocity ($r,\theta$)-slices of the mean flow field behind one stator segment ($x/c=0.32$).}
\end{center}
\end{figure}

%results




